Training Zero-Shot Generalizable End-to-End Task-Oriented Dialog System Without Turn-level Dialog Annotations

Task-oriented dialogue (TOD) systems enable users to achieve their goals through natural language interactions. Traditionally, these systems have relied on turn-level manually annotated metadata, such as dialogue states and policy annotations, which are expensive, time-consuming, and often inconsistent or error-prone. This dependence limits the potential to leverage vast amounts of readily available conversational data for training TOD systems. Additionally, a critical challenge in TOD system design is determining when and how to access and integrate information from external sources. Current approaches typically expect this information to be provided alongside the dialogue context, rather than learning to identify and retrieve it autonomously. While pre-trained large language models (LLMs) have been used to develop TOD systems, their potential to train such systems without laborious annotations remains largely unexplored. This work employs multi-task instruction fine-tuning to create more efficient and scalable TOD systems that can effectively leverage natural language conversational data without manual annotations, while autonomously managing external information retrieval. Our extensive experimental evaluations, using three diverse TOD datasets and three LLMs of varying sizes, demonstrate that our approach can generalize to new, unseen domains. Notably, our approach outperforms both state-of-the-art models trained on annotated data and billion-scale parameter off-the-shelf ChatGPT models.

==> my_files/map.tex <==
\begin{itemize}

\item \textbf{Intro}
\item what is tod
\item existing approaches use manual metadata to predict dst, action and response
\item some approaches add additional overhead to track state, decide policies.
\item expensive, error prone, thus making it limited.
\item goal of tod system: system response and api query
\item api call information added to metadata
\item real system needs to understand when to communicate with external sources
\item our approach: remove annotations, api call integral task
\item detailed explanation of different tasks in tod: retrieval, slot filling, api call, response
\item comparison on multiple datasets with different model types, sizes, chatgpt

\item \textbf{Method}
\item Data prep
\item API call, Multi
\item Retrieval, slot fill, response
\item Model instruction fine-tuning
\item prompt: schema, dialog history, task instruction
\item conditional generation

\item \textbf{Experiments}
\item Datasets, sgd, sgd-x, bitod, ketod
\item Metrics: gleu, bleu, api call

\item \textbf{Results}
\item SGD results with different models
\item Compare our best model with existing models

\item \textbf{Conclusion}
\item Summarize method
\item advantages of method
\item key results


\end{itemize}


